Model Predictive Control for Signal Temporal Logic Specification

We present a mathematical programming-based method for model predictive control of cyber-physical systems subject to signal temporal logic (STL) specifications. We describe the use of STL to specify a wide range of properties of these systems, including safety, response and bounded liveness. For synthesis, we encode STL specifications as mixed integer-linear constraints on the system variables in the optimization problem at each step of a receding horizon control framework. We prove correctness of our algorithms, and present experimental results for controller synthesis for building energy and climate control.

==> lasso.tex <==
\subsection{Finite Trajectory Parametrization}
%This aspect of our approach mirrors the approach used in bounded model checking of LTL formulas using SAT solvers \cite{BiereCCZ99}. A similar approach was recently used for the control of dynamical systems from linear temporal logic specifications in \cite{WolffTM14}. 
The notation used in this paper follows that of \cite{BiereHJLS06} and \cite{WolffTM14}, but is the first to extend it to support STL specifications. 
To allow interpretation of the STL specification over infinite sequences of states, an infinite sequence is represented using a finite number states forming a sequence consisting of a prefix and a loop -- we call this a ``lasso'' parametrization of the trajectory. Note that this added structure, enforcing that the trajectory eventually be periodic, may render our approach incomplete for some systems of the form (\ref{eq:model}) with an infinite state space.

After parametrizing an infinite trajectory by a finite, ``lasso-shaped'' form, 
%In order to specify properties of infinite executions of this finite parametrized trajectory, we will enforce a lasso shape on this finite sequence, requiring a loop that makes some eventual portion of the trajectory periodic. 
we will encode the STL formula as mixed integer-linear constraints on this finite form. The constraints from the system model are also included as part of the optimization problem. This allows Problem \ref{prob:stl} to be solved using a mixed-integer linear program (MILP) solver, which, although NP-hard, can be solved in practice for large problems using modern solvers with sophisticated search heuristics.  

We now present some definitions that are common to most approaches based on bounded model checking. 

\begin{definition} 
A run $\bf x$ is a \emph{$(N,l)$-loop} if $${\bf x} = (x_0x_1...x_{l-1})(x_l...x_N)^\omega,$$ such that $0 < l \le N$ and $x_{l-1} = x_N$, where $(\sigma)^\omega$ denotes infinite repetition of sequence $\sigma$.
\end{definition}

\begin{definition} 
Given a run $\bf x$ and a bound $N \in \mathbb{N}$, \emph{$\bf x$ finitely satisfies $\varphi$} (denoted ${\mathbf x} \models_N \varphi$) if and only if $\bf x$ is a $(N-l)$-loop for some $0 < l \le N$ and $({\bf x},0) \models \varphi$
\end{definition}

We propose to solve Problem \ref{prob:stl} by replacing ${\bf x}(x_0, {\bf u}) \models \varphi$ with ${\bf x}(x_0, {\bf u}) \models_N \varphi$, where $N$ is the length of the lasso parametrization. To do so, we build a set of MILP constraints that is satisfiable if and only if there exists a trajectory of length $N$ that finitely satisfies $\varphi$. The satisfiability of these constraints can be checked using a MILP solver, which also yields a solution to the constraints when feasible. 
%This solution gives us the control input $\bf u$ desired.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "root"
%%% End: 

